Fair Representation: Guaranteeing Approximate Multiple Group Fairness for Unknown Tasks

Motivated by scenarios where data is used for diverse prediction tasks, we study whether fair representation can be used to guarantee fairness for unknown tasks and for multiple fairness notions simultaneously. We consider seven group fairness notions that cover the concepts of independence, separation, and calibration. Against the backdrop of the fairness impossibility results, we explore approximate fairness. We prove that, although fair representation might not guarantee fairness for all prediction tasks, it does guarantee fairness for an important subset of tasks -- the tasks for which the representation is discriminative. Specifically, all seven group fairness notions are linearly controlled by fairness and discriminativeness of the representation. When an incompatibility exists between different fairness notions, fair and discriminative representation hits the sweet spot that approximately satisfies all notions. Motivated by our theoretical findings, we propose to learn both fair and discriminative representations using pretext loss which self-supervises learning, and Maximum Mean Discrepancy as a fair regularizer. Experiments on tabular, image, and face datasets show that using the learned representation, downstream predictions that we are unaware of when learning the representation indeed become fairer for seven group fairness notions, and the fairness guarantees computed from our theoretical results are all valid.

==> depd/fig_Adult_comparison.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.4\columnwidth}
        \centering
        \includegraphics[height=3.1cm]{Adult_compare_existing_methods_white.pdf}
        \caption{}
        \label{fig:comparison_Adult}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.59\columnwidth}
         \centering
         \includegraphics[height=3.1cm]{MPI3D_compare_existing_methods_white.pdf}
         \caption{}
         \label{fig:comparison_MPI3D}
     \end{subfigure}
    \caption{Comparison of our approach and existing fair representation learning methods on Adult (a) and uncorrelated MPI3D (b).
    We report the averaged PD coefficient for MPI3D because multiple target attributes are posed.
    Different markers of the same method correspond to different hyperparameters.
    We report the Pareto front for each method for fair comparison.
    Std is omitted for clarity.
    Complete results are reported in the supplementary material.
    }
    \label{fig:comparison}
    \vspace{-3ex}
\end{figure}

==> depd/fig_MPI3D_comparison.tex <==
\begin{figure}[!t]
    \includegraphics[width=.92\linewidth]{MPI3D_compare_existing_methods_white.pdf}
    \caption{Comparison of our approach and existing private representation learning methods on uncorrelated MPI3D dataset. Discriminativeness is the mean Balanced Accuracy (BA) of three target attributes, shape, size, and background color. Privacy is the BA of the sensitive attribute color. Std is omitted for clarity.}
    \label{fig:MPI3D_comparison}
    \vspace{-1ex}
\end{figure}

==> depd/fig_guarantees.tex <==

\begin{figure}[!t]
    \centering
    \begin{minipage}{1.0\linewidth} % <-- adjust this for resize
        \begin{minipage}{0.16\linewidth}
            \begin{minipage}[t][0.2\textwidth][t]{1.0\textwidth} \centerline{DOpp}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=1.8cm]{guarantees_blue/o1_1.pdf}}  \end{minipage}
            % \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o1_2.pdf}}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o1_3.pdf}}  \end{minipage}
        \end{minipage}
        \begin{minipage}{0.16\linewidth}
            \begin{minipage}[t][0.2\textwidth][t]{1.0\textwidth} \centerline{DR}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o2_1.pdf}}  \end{minipage}
            % \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o2_2.pdf}}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o2_3.pdf}}  \end{minipage}
        \end{minipage}
        \begin{minipage}{0.16\linewidth}
            \begin{minipage}[t][0.2\textwidth][t]{1.0\textwidth} \centerline{DOdds}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o3_1.pdf}}  \end{minipage}
            % \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o3_2.pdf}}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o3_3.pdf}}  \end{minipage}
        \end{minipage}
        \begin{minipage}{0.285\linewidth}
            \begin{minipage}[t][0.166\textwidth][t]{1.0\textwidth} \centerline{DWC}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o4_1.pdf}}  \end{minipage}
            % \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o4_2.pdf}}  \end{minipage}
            \begin{minipage}{1.0\textwidth} \centerline{\includegraphics[height=2.1cm]{guarantees_blue/o4_3.pdf}}  \end{minipage}
        \end{minipage}
    \end{minipage} 
    %
    % \setlength\tabcolsep{1pt}
    % \begin{tabular}{c c c c c}
    %     DOpp & DR & DOdds & DWC \\
    %     \includegraphics[height=14.5ex]{guarantees_blue/o1_1.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o2_1.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o3_1.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o4_1.pdf} \\
    %     \includegraphics[height=14.5ex]{guarantees_blue/o1_2.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o2_2.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o3_2.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o4_2.pdf} \\
    %     \includegraphics[height=14.5ex]{guarantees_blue/o1_3.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o2_3.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o3_3.pdf}&
    %     \includegraphics[height=14.5ex]{guarantees_blue/o4_3.pdf} \\
    % \end{tabular}
    \caption{Fairness guarantees of DOpp, DR, DOdds, and DWC w.r.t. different PC (x-axis) and PD (y-axis) coefficients. Rows correspond to different population base rates: $a=b=r=\!.5$ [top] and $a=\!.1$, $b=\!.3$, $r=\!.5$ [bottom]. Lower values indicate better fairness guarantees. The region above the red line denotes fairness value $< 0.5$. The gray area denotes the infeasible region, where the PC and PD coefficients are impossible under the give base rates.} \label{fig:guarantees}
    \vspace{-1ex}
\end{figure}

==> depd/fig_problem_overview.tex <==
\definecolor{yellow}{HTML}{FFB366}
\definecolor{blue}{HTML}{66B2FF}
\definecolor{green}{HTML}{00994D}
\definecolor{red}{HTML}{EA5E5E}

\begin{figure}[!t]
    \centering
    % \includegraphics[trim=18px 0 18px 0,clip,width=1.0\linewidth]{problem_overview.pdf}
    \includegraphics[width=1.0\linewidth]{problem_overview.pdf}
    \caption{\label{fig:problem_overview}
        An illustration of the problem setting.
        The service provider transforms multimedia data provided by users into new representations and vendors apply classifiers on the MM data representation.
        The service provider additionally wants to guarantee fairness for vendors' predictions.
        }
    \vspace{-3,5ex}
\end{figure}

==> depd/fig_tradeoff.tex <==
\begin{figure}[!t]
    \centering
    \renewcommand{\arraystretch}{0.5}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c c c c}
        {$(.4,.6,.5)$} & {$(.3,.7,.5)$} & {$(.2,.8,.5)$} & {$(.2,.8,.2)$} \\
        \includegraphics[height=15ex]{tradeoff/tradeoff_1.pdf}&
        \includegraphics[height=15ex]{tradeoff/tradeoff_2.pdf}&
        \includegraphics[height=15ex]{tradeoff/tradeoff_3.pdf}&
        \includegraphics[height=15ex]{tradeoff/tradeoff_4.pdf}
    \end{tabular}
    \caption{\label{fig:tradeoff} The privacy-discriminativeness tradeoff from Theorem~\ref{thm:tradeoff} (infeasible above the red solid line) and grid search (infeasible in the gray region) for four different base rate configurations ($(a,b,r)$ denoted on top). The red dash line denotes the worst scenario tradeoff. Theorem~\ref{thm:tradeoff} is close to the tradeoff found using grid search, which is tight up to grid size (0.05).} 
\end{figure}

==> depd/tab_ablation_Fourier.tex <==
\begin{table}[t]
    % \vspace{-1ex}
    \centering
    \caption{Ablation with Approximated MMD$^2$.}% (Gaussian kernel).}
    \label{tab:ablation_Fourier}
    \adjustbox{width=1\columnwidth}{
    \begin{tabular}{l c c c c | c}
    \toprule
    \# basis functions  & 256 & 512 & 1024 & \textbf{exact} \\ \midrule
    Color (\%, $\downarrow$)
    % & 59.2{\small\textcolor{gray}{$\pm$9.0}}      
    & 52.1{\small\textcolor{gray}{$\pm$2.6}}  
    & 53.6{\small\textcolor{gray}{$\pm$3.4}}  
    & 53.4{\small\textcolor{gray}{$\pm$5.1}}
    & 50.7{\small\textcolor{gray}{$\pm$1.2}}\\
    Shape (\%, $\uparrow$)
    % & 54.9{\small\textcolor{gray}{$\pm$3.7}}      
    & 51.3{\small\textcolor{gray}{$\pm$1.0}}
    & 52.9{\small\textcolor{gray}{$\pm$3.2}}  
    & 52.9{\small\textcolor{gray}{$\pm$3.1}}
    & 84.6\small{\textcolor{gray}{$\pm$3.0}}\\
    Size (\%, $\uparrow$)
    % & 54.9{\small\textcolor{gray}{$\pm$3.7}}      
    & 52.1{\small\textcolor{gray}{$\pm$1.6}}
    & 54.4{\small\textcolor{gray}{$\pm$3.7}}  
    & 52.1{\small\textcolor{gray}{$\pm$3.1}}
    & 86.8\small{\textcolor{gray}{$\pm$3.4}}\\
    Bkgd color (\%, $\uparrow$)
    % & 54.9{\small\textcolor{gray}{$\pm$3.7}}      
    & 56.4{\small\textcolor{gray}{$\pm$9.6}}
    & 60.4{\small\textcolor{gray}{$\pm$13.1}}  
    & 53.5{\small\textcolor{gray}{$\pm$5.6}}
    & 96.1\small{\textcolor{gray}{$\pm$4.2}}\\ \bottomrule
    \end{tabular}}
\end{table}


==> depd/tab_ablation_biased.tex <==
\begin{table}[t]
    \vspace{-1ex}
    \centering
    \caption{Ablation with Biased/Unbiased MMD$^2$ Estimates.}
    \label{tab:ablation_biased}
    \adjustbox{width=1\columnwidth}{
    \begin{tabular}{lccccc}
    \toprule
    \multirow{2}{*}{}\hspace{16ex} & \multicolumn{2}{c}{$k_{G}$}    & & \multicolumn{2}{c}{$k_{RQ}$} \\
    \cmidrule{2-3} \cmidrule{5-6} 
                                   & biased                & \textbf{unbiased}                      & & biased                & \textbf{unbiased}                       \\ \midrule
    Color (\%, $\downarrow$)     
    & 51.7\small{\textcolor{gray}{$\pm$3.2}}  
    & 50.5\small{\textcolor{gray}{$\pm$0.7}} 
    & & 53.4\small{\textcolor{gray}{$\pm$3.4}}  
    & 50.7\small{\textcolor{gray}{$\pm$1.2}}  \\
    Shape (\%, $\uparrow$)         
    & 58.8\small{\textcolor{gray}{$\pm$9.4}}  
    & 84.4\small{\textcolor{gray}{$\pm$2.6}} 
    & & 69.4\small{\textcolor{gray}{$\pm$10.3}}  
    & 84.6\small{\textcolor{gray}{$\pm$3.0}}  \\
    Size (\%, $\uparrow$)         
    & 59.2\small{\textcolor{gray}{$\pm$10.8}}  
    & 87.0\small{\textcolor{gray}{$\pm$2.2}} 
    & & 71.1\small{\textcolor{gray}{$\pm$12.1}}  
    & 86.8\small{\textcolor{gray}{$\pm$3.4}}  \\
    Bkgd color (\%, $\uparrow$)         
    & 64.2\small{\textcolor{gray}{$\pm$16.3}}  
    & 98.2\small{\textcolor{gray}{$\pm$1.0}} 
    & & 82.0\small{\textcolor{gray}{$\pm$15.6}}  
    & 96.1\small{\textcolor{gray}{$\pm$4.2}}  \\ \bottomrule
    \end{tabular}}
    \vspace{-2ex}
\end{table}


==> depd/tab_ablation_diff_predictors.tex <==
\begin{table}[h]
    \centering
    \caption{Ablation Study with Different Adversarial Models. 
    % The Representations are Learned on Uncorrelated MPI3D Dataset using the Proposed Approach.
    Balanced Accuracy (\%) is Reported.
    The Random Prediction Baseline is $50\%$.}
    \label{tab:ablation_diff_predictors}
    \adjustbox{width=1\columnwidth}{
    \begin{tabular}{l c c c l}
    \toprule
    \hspace{25ex} & color & shape & size & bkgd color              \\
    \midrule
    Gaussian Naive Bayes   & 50.3\small{\textcolor{gray}{$\pm$0.6}}  & 58.3\small{\textcolor{gray}{$\pm$4.3}} & 58.0\small{\textcolor{gray}{$\pm$4.6}}  & 61.9\small{\textcolor{gray}{$\pm$11.4}}  \\
    Linear Regression   & 50.6\small{\textcolor{gray}{$\pm$0.9}}  & 68.8\small{\textcolor{gray}{$\pm$2.7}} & 71.1\small{\textcolor{gray}{$\pm$4.5}}  & 75.2\small{\textcolor{gray}{$\pm$12.4}}  \\
    Decision Tree   & 50.0\small{\textcolor{gray}{$\pm$0.9}}  & 74.4\small{\textcolor{gray}{$\pm$2.9}} & 76.6\small{\textcolor{gray}{$\pm$4.2}}  & 82.8\small{\textcolor{gray}{$\pm$10.8}}  \\
    Random Forest   & 49.6\small{\textcolor{gray}{$\pm$0.8}}  & 79.2\small{\textcolor{gray}{$\pm$2.8}} & 81.8\small{\textcolor{gray}{$\pm$4.2}}  & 86.5\small{\textcolor{gray}{$\pm$10.3}}  \\
    Support Vector Machine   & 50.6\small{\textcolor{gray}{$\pm$0.5}}  & 75.8\small{\textcolor{gray}{$\pm$3.6}} & 78.9\small{\textcolor{gray}{$\pm$6.4}}  & 87.6\small{\textcolor{gray}{$\pm$10.5}}  \\
    5-Nearest Neighbors   & 49.4\small{\textcolor{gray}{$\pm$1.0}}  & 79.0\small{\textcolor{gray}{$\pm$3.4}} & 82.1\small{\textcolor{gray}{$\pm$5.1}}  & 84.3\small{\textcolor{gray}{$\pm$12.7}}  \\
    \midrule
    7-Net (width $8\times$) (ours)   & 50.7\small{\textcolor{gray}{$\pm$1.2}}  & 84.6\small{\textcolor{gray}{$\pm$3.0}} & 86.8\small{\textcolor{gray}{$\pm$3.4}}  & 96.1\small{\textcolor{gray}{$\pm$4.2}}  \\
    7-Net (width $16\times$)   & 51.0\small{\textcolor{gray}{$\pm$1.3}}  & 85.4\small{\textcolor{gray}{$\pm$2.9}} & 87.9\small{\textcolor{gray}{$\pm$3.3}}  & 96.6\small{\textcolor{gray}{$\pm$3.6}}  \\
    12-Net   & 50.9\small{\textcolor{gray}{$\pm$1.4}}  & 84.8\small{\textcolor{gray}{$\pm$3.0}} & 87.1\small{\textcolor{gray}{$\pm$3.6}}  & 96.3\small{\textcolor{gray}{$\pm$3.8}}  \\
    \bottomrule
    \end{tabular}}
    % \vspace{-3ex}
\end{table}


==> depd/tab_ablation_kernel.tex <==
\begin{table}[h]
    \vspace{-1ex}
    \centering
    \caption{Ablation with different kernels (Gaussian kernel $k_{G}$ and Ratioanl Quadratic kernel $k_{RQ}$) and different length scale $l$.}
    \label{tab:ablation_kernel}
    \begin{tabular}{l l c c c c c}
    \toprule
    & $l$      & 0.25 & 0.5 & 1 & 4 & 16 \\ \midrule
    % \multirow{2}{*}{\makecell{Privacy (\%, $\downarrow$)}} 
    \multirow{2}{*}{PC coef. ($\downarrow$) }& $k_{G}$  & .752\small{\textcolor{gray}{$\pm$.152}} & .302\small{\textcolor{gray}{$\pm$.044}} & \textbf{.010}\small{\textcolor{gray}{$\pm$.014}} & .024\small{\textcolor{gray}{$\pm$.020}} & .140\small{\textcolor{gray}{$\pm$.104}} \\ 
    \cmidrule{2-7} 
    & $k_{RQ}$ & .156\small{\textcolor{gray}{$\pm$.074}} & .152\small{\textcolor{gray}{$\pm$.044}} & \textbf{.014}\small{\textcolor{gray}{$\pm$.024}} & .024\small{\textcolor{gray}{$\pm$.020}} & .118\small{\textcolor{gray}{$\pm$.056}} \\
    \midrule 
    % \multirow{2}{*}{\makecell{Disc. (\%, $\uparrow$)}}    
    \multirow{2}{*}{PD coef. ($\downarrow$)} & $k_{G}$  & .490\small{\textcolor{gray}{$\pm$.024}} & .398\small{\textcolor{gray}{$\pm$.010}} & \textbf{.202}\small{\textcolor{gray}{$\pm$.028}} & .318\small{\textcolor{gray}{$\pm$.086}} & .324\small{\textcolor{gray}{$\pm$.108}} \\ 
    \cmidrule{2-7} 
    & $k_{RQ}$& .458\small{\textcolor{gray}{$\pm$.034}} & .294\small{\textcolor{gray}{$\pm$.038}} & \textbf{.218}\small{\textcolor{gray}{$\pm$.040}} & .308\small{\textcolor{gray}{$\pm$.100}} & .326\small{\textcolor{gray}{$\pm$.082}} \\ 
    \bottomrule
    \end{tabular}
\end{table}


==> depd/tab_ablation_lambda.tex <==
\begin{table}[h]
    \centering
    \caption{Ablation with weight $\lambda$ and shape parameter $\alpha$.}
    \label{tab:ablation_lambda}
    \begin{tabular}{l c c c c c}
    \toprule
    $\lambda$\hspace{13ex}  &  1e-1 & 1 & 1e1  & 1e2 & 1e3 \\ \midrule
    PC coef. ($\downarrow$)   & .216{\small\textcolor{gray}{$\pm$.042}}  & .020{\small\textcolor{gray}{$\pm$.018}} & .014{\small\textcolor{gray}{$\pm$.024}} & -.016{\small\textcolor{gray}{$\pm$.018}} & -.012{\small\textcolor{gray}{$\pm$.018}}  \\
    PD coef. ($\downarrow$)      &  .182{\small\textcolor{gray}{$\pm$.010}} & .186{\small\textcolor{gray}{$\pm$.008}}  & .218{\small\textcolor{gray}{$\pm$.040}}  & .224{\small\textcolor{gray}{$\pm$.036}} & .224{\small\textcolor{gray}{$\pm$.036}}  \\ \midrule
    \midrule
    $\alpha$ & 1 & 2 & 4 & 8 & 12 \\ \midrule
    PC coef. ($\downarrow$)   & .016{\small\textcolor{gray}{$\pm$.014}}  & .016{\small\textcolor{gray}{$\pm$.018}} & .014{\small\textcolor{gray}{$\pm$.024}} & .002{\small\textcolor{gray}{$\pm$.020}} & .008{\small\textcolor{gray}{$\pm$.016}}  \\
    PD coef. ($\downarrow$)      &  .226{\small\textcolor{gray}{$\pm$.044}} & .220{\small\textcolor{gray}{$\pm$.036}}  & .218{\small\textcolor{gray}{$\pm$.040}}  & .206{\small\textcolor{gray}{$\pm$.020}} & .198{\small\textcolor{gray}{$\pm$.020}}  \\ 
    \bottomrule
    \end{tabular}
\end{table}

